A Simple Parallel Implementation of Interaction Nets in Haskell

Due to their "inherent parallelism", interaction nets have since their introduction been considered as an attractive implementation mechanism for functional programming. We show that a simple highly-concurrent implementation in Haskell can achieve promising speed-ups on multiple cores.

==> eptcsdata.tex <==
\providecommand{\firstpage}{33}
\providecommand{\publicationstatus}{U. Dal Lago and R. Harmer (Eds.): Developments\\
in Computational Models 2014 (DCM 2014).\\
EPTCS 179, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.179.3}{10.4204/EPTCS.179.3}}
\pdfoutput=1

